Enabling Large Neural Networks on Tiny Microcontrollers with Swapping

Running neural networks (NNs) on microcontroller units (MCUs) is becoming increasingly important, but is very difficult due to the tiny SRAM size of MCU. Prior work proposes many algorithm-level techniques to reduce NN memory footprints, but all at the cost of sacrificing accuracy and generality, which disqualifies MCUs for many important use cases. We investigate a system solution for MCUs to execute NNs out of core: dynamically swapping NN data chunks between an MCU's tiny SRAM and its large, low-cost external flash. Out-of-core NNs on MCUs raise multiple concerns: execution slowdown, storage wear out, energy consumption, and data security. We present a study showing that none is a showstopper; the key benefit -- MCUs being able to run large NNs with full accuracy and generality -- triumphs the overheads. Our findings suggest that MCUs can play a much greater role in edge intelligence.

==> analysis.tex <==
% !TeX root = main.tex
\section{Analysis}
\subsection{How parameters affect swapping performance}
There are multiple parameters that affect the swapping performance, 
including SRAM size, NN's memory footprint, buffer size, the number of buffers.

Buffer sizes and the number of buffers affect swapping performance.
Larger buffer sizes leads to less IO traffic/time, and more buffers lead to high parallelism.
Given a SRAM size, there is a tradeoff between buffer sizes and the number of buffers.
If the buffer size is larger, then the number of buffers is smaller, and vice versa.
Larger buffer sizes can reduce overall IO traffic, but limit the parallelism.
Smaller buffer sizes can increase parallelism, but also increase overall IO traffic.

The choice of larger or smaller buffer size depends on the gap between SRAM size and NN's memory footprint.
If the gap is large, larger buffer size (less buffers) leads to better performance, where the benefit of less IO traffic overcomes parallelism.
If the gap is smaller, smaller buffer size (more buffers) leads to better performance, where the benefit of high parallelism overcomes the benefit of less IO traffic.


\begin{comment}
Today's SRAM size is small, but future MCU may have larger SRAM, so swapping is more promising.

What parametersafafasdf

How they affect each other: parallelism, IO
today’s hardware, parameter range
Findings…

What figures I need: one alexnet figures
content...
\end{comment}

==> discussion.tex <==
% !TeX root = main.tex
\section{Discussion}
%In previous section, we demonstrate it's feasible to using MicroSD for swapping to enable large NNs on MCUs with tiny SRAM.
%In this section, we discuss some challenges and corresponding solution to make swapping practical.
%We discuss the potential impact of our system-level solution on TinyML community.
In this section, we discuss how future hardware may affect the swapping solution, and how our system-level solution may impact TinyML community.
\begin{comment}
\subsection{Embedded AI Accelerators}
\begin{itemize}
	\item what's problem: sram still too small, swapping still needed
	\item is swapping slowdown small? accelerators are fast, IO cannot be hidden
	\item durability is not a problem either: write too few, write frequency is low
\end{itemize}
\end{comment}
\paragraph{Future Embedded Hardware}
\begin{comment}
\begin{itemize}
	\item Embedded AI accelerator: memory still small (512KB)
	\item Relative speed of compute and IO: IO will be the bottlenck in swapping. advance in storage is needed.
	\item is swapping still valid in future?
\end{itemize}
\end{comment}
Due to the mismatch between the high compute demand of NN and the low compute speed of MCU, 
many hardware vendors integrate AI accelerators on MCU devices, such as ARM Ethos-U55~\cite{ethos-u55} and MAX78000~\cite{max78000}.
These AI accelerators can speedup NN by more than 100$\times$, but their SRAM is till too small to run large models, e.g., 18-50 KB on Ethos-U55 and 128 KB on MAX78000. 
Swapping is still needed for them to run large NN models.

However, MicroSD's IO speed may not be able to catch up with AI accelerators' compute speed, so the IO is likely to become the bottleneck.
Therfore, we expect that new swapping media with high speed, low cost, and low energy consumption will be needed in the future.\note{shoot our own foot?}
 

\paragraph{Impact on TinyML Community} \Note{redundant. may cut}
\begin{comment}
\begin{itemize}
	\item precondition of impact: if swapping incurs zero/negligible slowdown on throughput
	\item system-level innovation makes algorithm-level engineering unneeded
	\item swapping may enable transfer/federated learning on MCU with zero/negligible slowdown at the first time
	\item significantly expand the possible AI application on tiny MCUs
	\item enable training on MCU
\end{itemize}
\end{comment}
Running ML applications on MCUs is an open challenge in TinyML community.
Most people are working on algorithm-level techniques, which are trying extremely hard to compress models as small as possible, of course, at the cost of sacrificing accuracy.
Different from them, we solve the problem in system-level, using MicroSD as a swapping media.
According to the analysis, our solution incurs zero/negligible performance slowdown, and most importantly, without losing accuracy.
Our system-level solution makes algorithm-level solution less needed, and it dramatically expands the scope of ML applications on tiny MCU devices.
It not only enables large NN inference on tiny MCU possible, but also enables training on tiny MCU possible.

\begin{comment}
\subsection{Future work}
\begin{itemize}
	\item programmability challenge: auto tiling + code generation
	\item latency too long: io-aware pruning
\end{itemize}
\end{comment}




==> fig-alexnet-perf.tex <==
\begin{figure}[t!]
\centering
    %\includegraphics[width=0.48\textwidth{}]{./figs/fake-alexnet.jpeg}
    \includegraphics[width=0.48\textwidth{}]{./figs/plot/alexnet-perf/alexnet-128k.pdf}
    \caption{1. Compute-bound Conv: long compute time, IO can be hidden by compute. 2. IO-bound FC: long IO time, cannot be hidden by compute. 3. Others Relu/Maxpool: IO and compute time is negligible.}
    %\vspace{-2pt}		% use as needed
    \label{fig:alexnet-128k}
\end{figure}


==> fig-energy.tex <==
\begin{figure}[t!]
%\begin{figure*}
\centering
    \includegraphics[width=0.45\textwidth{}]{./figs/plot/energy/energy.pdf} 
    \caption{Per-frame energy consumption of NNs: to show that swapping won't increase energy too much (compute only vs. compute+io)}
    %\vspace{-15pt}		% use as needed
    \label{fig:energy}
%\end{figure*}
\end{figure}


==> fig-hetero-mcu-sram.tex <==

\begin{table}[t!]
\centering
    \includegraphics[width=0.48\textwidth{}]{./figs/hetero-mcu-sram} 
    \caption{Core, SRAM size, and cost of typical MCUs.}
    %\vspace{-2pt}		% use as needed
    \label{tab:hetero-mcu-sram}
\end{table}



==> fig-iob-cpb.tex <==
\begin{figure}[t!]
\centering
    %\includegraphics[width=0.48\textwidth{}]{./figs/fake-alexnet.jpeg}
    \includegraphics[width=0.48\textwidth{}]{./figs/plot/iob-cpb/iob-cpb.pdf}
    \caption{(1) Delay of an NN is determined by compute time of compute-bound layers and IO time of IO-bound layers. (2) Pipeline parallelism to reduce throughput loss: IO in one frame can be hidden by compute in another frame.}
    %\vspace{-2pt}		% use as needed
    \label{fig:iob-cpb}
\end{figure}


==> fig-latency.tex <==
\begin{figure}[t!]
%\begin{figure*}
\centering
    \includegraphics[width=0.45\textwidth{}]{./figs/plot/latency/latency.pdf} 
    \caption{Per-frame delay to show: (1) simple parallel scheduling can reduce latency a lot; (2) swapping with parallel scheduling won't increase latency much}
    %\vspace{-15pt}		% use as needed
    \label{fig:latency}
%\end{figure*}
\end{figure}


==> fig-mobilenet-perf.tex <==
\begin{figure}[t!]
\centering
    %\includegraphics[width=0.48\textwidth{}]{./figs/fake-alexnet.jpeg}
    \includegraphics[width=0.48\textwidth{}]{./figs/plot/mobilenet-perf/mobilenet-224-1-128k.pdf}
    \caption{Mobilenet: 1. 27 Convs vs. 1 FC. 2. Compute time of Convs > IO time of FCs}
    %\vspace{-2pt}		% use as needed
    \label{fig:mobilenet-224-1-128k}
\end{figure}


==> fig-sd-liftime.tex <==

\begin{table}[t!]
%\begin{table}[htb]
\centering
    \includegraphics[width=0.47\textwidth{}]{./figs/sd-lifetime.pdf} 
    \caption{The lifetime of a 32GB SD with swapping}
    %\vspace{-10pt}		% use as needed
    \label{tab:sd-lifetime}
\end{table}



==> fig-stm32f746ng.tex <==

\begin{table}[t!]
\centering
    \includegraphics[width=0.48\textwidth{}]{./figs/stm32f746ng.pdf} 
    \caption{STM32F746NG-Disco board used in evaluation. \textbf{To be deleted}}
    \vspace{-5pt}		% use as needed
    \label{tab:stm32f746ng}
\end{table}



==> fig-throughput.tex <==
\begin{figure}[t!]
%\begin{figure*}
\centering
    \includegraphics[width=0.45\textwidth{}]{./figs/plot/throughput/throughput.pdf} 
    \caption{NN throughputs: (1) swapping with parallel scheduling won't decrease throughput much (compute only vs. io/compute in parallel), (2) simple parallel algorithm can increase throughput a lot (io/compute parallel vs. sequencial)}
    %\vspace{-15pt}		% use as needed
    \label{fig:throughput}
%\end{figure*}
\end{figure}


==> fig-vgg-perf.tex <==
\begin{figure}[t!]
\centering
    %\includegraphics[width=0.48\textwidth{}]{./figs/fake-alexnet.jpeg}
    \includegraphics[width=0.48\textwidth{}]{./figs/plot/vgg-perf/vgg-128k.pdf}
    \caption{VGG16: 1. 13 Convs vs. 3 FC. 2. Compute time of Convs > IO time of FCs}
    %\vspace{-2pt}		% use as needed
    \label{fig:vgg-128k}
\end{figure}


==> intro-hongyu.tex <==
% !TeX root = main.tex
%-------------------------------------------------------------------------------
\section{Introduction}
%-------------------------------------------------------------------------------

\Note{this paragraph can be gone. Instead, state several concrete use cases of NN on MCU.}
(\note{gone: NO. have to convince distributed people in ATC to understand why tiny devices have future and why it's important to run ML on them locally})
There are 250 billion microcontroller units (MCU) in the world today, and the annual shipment volume will grow to 38.2 billion by 2023~\cite{tinymlopt}. 
Driven by new applications, such as smart cities, smart manufacture, and precision agriculture, running machine learning (ML) on these tiny MCUs (TinyML) has a giant opportunity. 
Running ML on MCU locally is attractive,
because it has low power consumption (\note{unique}), reserves data privacy, saves network bandwidth, and performs ML tasks in offline settings.
\Note{these benefits are not unique to MCUs}  (\note{NO. Not necessarily to be unique. People have asked many times for the question why run NN on edge/MCU locally, instead of cloud. we must answer it here})
%ref: MCUNet: Tiny Deep Learning on IoT Devices
For instance, Nuru app helps farmers detect diseases in plants just by taking a picture of it by running ML models on MCU devices deployed in farms, so there is no need for internet connection. This is a crutial requirement for remote farmers since they might not have proper internet connection in their place
~\cite{nuruai,introtinyml}. Most importantly, MCUs are cheap (a few \$), so it's affordable for farmers to deploy hundreds or thousands of MCUs to their farms.
(\note{concrete use case: YES. Nuru app above})

\input{fig-models-accuracy-memory}
\input{fig-hetero-mcu-sram}

However, the top resource constraint for ML on MCU is memory size.
ML relies on large memory footprint for accuracy, 
which is at odds with MCU's small memory (SRAM).
\Note{``top'' too strong. why CPU speed is less important?} (\note{NO. we address memory problem, but not speed problem. discussing speed here is confusing})
The size gap between them could be a few orders of magnitude, which makes running ML on MCU very difficult.
Figure~\ref{fig:hetero-mcu-sram} shows some typical MCUs, whose SRAM sizes range from a few KB to hundreds KB. 
\Note{there exist MCUs with MBs of SRAM. Shouldn't dismiss them so easily}
(\note{YES. next sentence})
Although it's possible to have a few MBs of SRAM, the cost will be too high. \Note{how high? Why not just say the MCU SRAM is a few KB to a few MB?}
However, typical ML models require at least tens/hundreds MB of memory, e.g., 63MB for AlexNet (with quantization), 54MB for MobileNet, and 236MB for VGG~\cite{memfootprint}, 
which are 3 orders of magnitude larger than SRAM sizes.
\Note{Missing obvious discussion on per-layer memory footprints, and weights (RO) vs feature maps (RW) memory}
(\note{YES. next sentence})
What's even worse, a single layer's memory footprint, which includes input/output feature maps and weights parameters, is larger than SRAM size.
For instance, 8 (Conv\&FC) of 13 layers in AlexNet have memory footprint that is larger than 1 MB (with quantization).
\Note{AlexNet too small to be a good example? 1MB is not too large? Diff RW and RO mem}


%Prior work has come up with various techniques to reduce the memory footprint of ML models
The tradeoffs between model memory and model accuracy has been explored by prior work, 
such as compression~\cite{prune, deepcompression, prunefilter},  quantization~\cite{limitedprecision}, designing new efficient network~\cite{bmxnet}, inventing new architecture search algorithm (MCNet~\cite{lin2020mcunet}).
However, all these techniques sacrifice accuracy or model generality as the cost,
and most models still cannot fit into MCU's SRAM after applying these techniques.
\Note{just say the norm has been exploring the tradeoffs between model accuracy vs model memory}
(\note{YES. above})
As Figure~\ref{fig:models-accuracy-memory} shows,
most models (even their compressed versions) cannot fit into SRAM.
When models are compressed small enough to fit SRAM, the accuracy loss is substantial. For example, the accuracy of VGG (32x32) drops from 89\% to 52\% after fitting into 100 KB SRAM, but the accuracy is too low to be usable.
%and may only suite specific tasks, like hot word recognition).
%For instance, Deep Compression~\cite{deepcompression} can compress VGG-16-224 model by 49x from 552 MB to 11.3 MB, which still cannot fit into MCU SRAM. 
Such drawbacks disqualify many use cases where large ML models (albeit slow speed) with high accuracy are a must, 
for instances, profiling and object counting~\cite{xu2020approximate}. \Note{need a few more. be more systematic} (\note{YES. but how systematic?})

We revisit an idea: using external flash storage, microSD, as a swapping space for NN inference \textit{without losing accuracy}. \Note{``w/o losing accuracy.'' -- really do not have to argue for this} (\note{NO. this is the KEY advantage over algorithm-level solutions. If don't argue for this, what's the advantage? why not just use compression? why use swapping?})
\Note{the advantage is to allow large memory footprint w/o low overhead. Our proposal and compression are NOT mutually exclusive; they are compatible. For instance, people can compress less. I don't see any point aruging against compression.}
Swapping to flash storage has been explored on MCU in the context of sensor networks. %[\note{cite}]. 

\Note{the following discussion unnecessary; weak.}
(\note{NO. swapping is well known. we must state clearly what is not new (swapping), and what is not (swapping for ML workload)})
\Note{``Our work is valuable because we did apply an old techinuqe to a new context'' -- this is weak. You just need to show what are the new insights. The following sentences do not carry too much info. They are likely to be deleted because of space limit.}
However, it is never examined for ML workload which is a new compute paradigm that is always on, intensive, and approximate, 
and for recent embedded hardware which has larger and cheaper external storage.
Is it feasible and practical for enabling large NNs on MCUs?
Are there any new opportunities and challenges? 
Many questions are unanswered.

In this paper, we contribute a thorough study on the feasibility of swapping by answering the following questions:

\Note{A few key insights should be highlighted, e.g. workloads of a NN (Conv vs FC), the relative speeds of CPU and IO; mostly-read IO workloads --> insignificant durability loss; CPU/IO parallelism at various levels could help}

\Note{some interesting and non-trivial findings, e.g. exploiting parallelism, should be highlighted. Some key numbers, e.g. XX MCU can run YY model at ZZ speed, should be stated}

\Note{state conclusions; summarize findings}

\note{YES. see contributions below}

\st{(1) Why use MicroSD, instead of DRAM? 
Our analysis shows that MicroSD has advantages over DRAM in terms of cost, capacity, and energy consumption.}
\Note{this is about cost analysis. not quite a research problem.}
(\note{YES. delete then})

(2) Would continuous swapping adversely affect MCU lifetime, leading to early wear out? 
Our analysis shows that durability loss is negligible, and the lifetime of MicroSD would be several or tens of years.

(3) Would swapping slow down NN inference much? Our analysis shows that the slowdown is as low as XXX, after we overlap the compute and IO.

(4) Would swapping consume much energy? Our estimation and measurement show that the swapping won't increase energy consumption much, compared to the overall system's energy consumption.

\Note{security?} \note{YES. below}

(5) Is there security issue? Yes, but data can be encrypted/decrypted by accelerators on MCU, which is very fast.
 
\Note{fault tolerance?} \note{YES. below}

(6) What if disk failures happen? Yts, but can be easy addressed by writing each block twice to MicroSD.

%(5) Are there any other challenges in swapping data to MicroSD?
%(5) Is it practical to deploy NNs with swapping in real world?We analyze the potential problems in programmability, MicroSD failures, and security, then conclude these problems can be easily addressed.
(7) Is it practical to implement swapping on MCUs? Yes. it's an open challenge, and is addressable.

\Note{there should be a contribution paragraph} \note{YES. see contributions below}
\st{
Our analysis demonstrates 
it's feasible and practical to enable large ML models on MCUs with tiny SRAM \textit{without losing accuracy} by swapping data to external MicroSD.
It's the first time that a full model with hundreds-of-MB memory footprint can run a tiny MCU with hundreds-of-KB SRAM (gap is 3 orders of magnitude).
It dramatically expands the scope of AI applications on tiny devices.}

\note{In this paper, we make the following contributions:}

\Note{contributions should be concise. Too long. Insights/contents shall move up.}

(1) we contribute a through feasibility study on the idea of swapping data to MicroSD to enable large NN models on MCUs with tiny SRAM. Our answer is that it's feasible and we have the following insights:
\begin{itemize}
	\item MicroSD durability loss is not a big deal.
	\item extra power consumption due to swapping is low.
\end{itemize}

(2) we contribute a detailed analysis for CNN workloads on MCU with MicroSD as swapping media. We have the following findings:
\begin{itemize}

\item CNNs are mostly-read IO workloads, which incurs insignificant/negligible durability loss on MicroSD.

\note{details: can be cut}
Read IO comes from loading input feature maps and weight parameters from MicroSD to SRAM, and write IO only comes from storing output feature maps to MicroSD.
The total size of input feature maps and weight parameters is much larger than the size of output feature maps, so the most IO time is spent on reading. \note
{add numbers}, e.g., for NN model has XX read IO and YY write IO, the lifetime of MicroSD can be SS.

\item 
The increased latency due to swapping is low after we exploit parallelism within each layer in a model to overlap their own IO and compute.
The decreased throughput due to swapping is low after we exploit parallelism across consecutive images/frames to overlap the compute of Convs and the IO of FCs.

\note{details: can be cut}
The execution time of a model is dominated by the compute time of Convs, and the IO time of FCs.
Convs have high compute complexity and relatively small amount of parameters, and MCU speed is low, so Convs execution time is dominated by compute.
FCs have large amount of weight parameters and relatively low compute complexity, and IO is slow, so FCs execution time is dominated by IO. 
Other layers, like Relu/Maxpool, have much lighter compute complexity and less parameters, so their execution time is negligible to the whole model's. \note{add numbers} e.g., XX MCU can run YY models at ZZ speed.
\end{itemize}

(3) we show the first time that a full model with hundreds-of-MB memory footprint can run a tiny MCU with hundreds-of-KB SRAM (gap is 3 orders of magnitude) without losing accuracy.
It dramatically expands the scope of AI applications on tiny devices.


==> power-consumption.tex <==

\begin{table}[t!]
\centering
    \includegraphics[width=0.48\textwidth{}]{./figs/power-consumption.pdf} 
    \caption{Power consumption measured on STM32F746NG-Disco with MicroSD}
    \vspace{-5pt}		% use as needed
    \label{tab:power-consumption}
\end{table}



==> schedule-algorithm.tex <==
% !TeX root = main.tex


\begin{algorithm}
\small
%\SetAlgoLine
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{NN architecture and SRAM size}
\Output{Tile sizes and parallel IO/compute sequence }

\texttt{\\} % add a blank line

%Let $tsIn[i]$, $tsWt[i]$, $tsOut[i]$= input, weight, output tile sizes of layer $i$\\
Let $Layers[L]$ = $L$ layers of an NN \\
Let $tnIn[L]$, $tnWt[L]$, $tnOut[L]$ = number of input, weight, and output tiles of NN layers \\

Let $\longrightarrow$ = add a task to graph to create dependency and update $inDegreeCounter$ for each task

\SetKwFunction{FBuildGraph}{BuildGraph}
    \SetKwProg{Fn}{Function}{:}{}
    \Fn{\FBuildGraph{$Layers$, $tIn$, $tWt$, $tOut$}}{
	    $G$ = empty graph \\
	    \For{$Layer \in Layers$} {
		    \For{$tin \in tIn$} {
				$IOTask\_ReadInput \longrightarrow G$; \\
				\For{$twt \in tWt$} {
					$IOTask\_ReadWt \longrightarrow G$; \\
					$ComputeTask \longrightarrow G$; \\
				}
		    }
		    $IOTask\_WriteOutput \longrightarrow G$;
	    }
	    Set the root IOTask to READY and insert into $ReadyIO$; \\
        \textbf{return} $G;$ 
}
\textbf{End Function}

%https://tex.stackexchange.com/questions/28868/how-do-i-add-a-blank-line-in-the-algorithmic-environment/509688
\texttt{\\} % add a blank line

Let $ReadyIO$ = a set of IO tasks in READY state \\
Let $ReadyCP$ = a set of Compute tasks in READY state \\
Let $SelectedIO$ = a set of IO tasks in Selected state \\
Let $SelectedCP$ = a set of compute tasks in Selected state \\
\SetKwFunction{FSelectTask}{SelectTask}
    \SetKwProg{Fn}{Function}{:}{}
    \Fn{\FSelectTask{$ReadyIO, ReadyCP, SelectedIO, SelectedCP$}}{
	    $CPT \longleftarrow$ empty minHeap for $M$ compute task candidates; \\
	    \For{$CPTask \in ReadyCP$} {
			update $CPT$ based on CPTask's time stamp;
	    }
	    $CPTime$ = time sum of tasks in $SetCP$; \\
		$M$ Compute tasks in $CPT \longrightarrow ReadyCP$; \\
		
		\texttt{\\}
		
		$IOT \longleftarrow$ empty minHeap for IO tasks candidates; \\
		\For{$IOTask \in ReadyIO$} {
			update $IOT$ based on IOTask's time stamp;
		}
		select $N$ IO tasks with smaller time stamps in $IOT$: whose time sum <= $CPTime$; \\
		$N$ Compute tasks $\longrightarrow ReadyIO$;	
}
\textbf{End Function}

\texttt{\\}

\SetKwFunction{FScheduleTask}{ScheduleTask}
    \SetKwProg{Fn}{Function}{:}{}
    \Fn{\FScheduleTask{$SelectedIO, SelectedCP$}}{
	
	Decide the execution orders of IO/compute tasks to avoid MCU/IO idling; // explain why order matters\\
	
	\For{$IOTask \in SelectedIO$} {
		execute the tasks; \\
		\For{$nextt \in$ successors of $IOTask$} {
			drops the $inDegreeCounter$ of $nextt$ by 1; \\
			\If {$inDegreeCounter$ of $nextt$ == 0} {
				$nextt \longrightarrow ReadyIO$ or $ReadyCP$;
			}
		}
	}
	
	\For{$CPTask \in SelectedCP$} {
		execute the tasks; \\
		\For{$nextt \in$ successors of $CPTask$} {
			drops the $inDegreeCounter$ of $nextt$ by 1; \\
			\If {$inDegreeCounter$ of $nextt$ == 0} {
				$nextt \longrightarrow ReadyIO$ or $ReadyCP$;
			}
		}
	}
}
\textbf{End Function}

\caption{Scheduling IO/compute tasks in parallel}
\label{algo:scheduler}
\end{algorithm}



% how to use function
% https://tex.stackexchange.com/questions/403823/how-to-use-function-in-latex-algorithm
\begin{comment}
\begin{algorithm}[H]
\SetAlgoLined
\DontPrintSemicolon
\KwIn{$ F $\Comment*[r]{List of Sensitive Terms}}    
\KwOut{$ S^{*} $ \Comment*[r]{Negation Excluded List}}

    \SetKwFunction{FMain}{NegationDetection}
    \SetKwProg{Fn}{Function}{:}{}
    \Fn{\FMain{$F$}}{
        $ S^{*}  \longleftarrow F $;    

        \ForEach{$ F \in NPs $}
        {\eIf{$ f_i = Negated $}
            {$ N \longleftarrow f_i;$}
            {$ S \longleftarrow f_i;$}

        }
        \textbf{return} $ S^{*}; $ 
}
\textbf{End Function}
\caption{Algorithm for Excluding the Negation}
\label{NagetionAlgo}
\end{algorithm}
\end{comment}

% How to use algorithm
% % https://www.overleaf.com/learn/latex/Algorithms
\begin{comment}
\begin{algorithm}
\SetAlgoLine
\KwResult{Write here the result }
 initialization\;
 \While{While condition}{
  instructions\;
  \eIf{condition}{
   instructions1\;
   instructions2\;
   }{
   instructions3\;
  }
 }
 \caption{How to write algorithms}
\end{algorithm}
\end{comment}

\begin{comment}
\let\oldnl\nl% Store \nl in \oldnl
\newcommand{\nonl}{\renewcommand{\nl}{\let\nl\oldnl}}% Remove line number for one line
%\vspace{-5pt}
\begin{algorithm}
	
\small
\caption{frame scheduling for each tagging pass}\label{algo:tagging}
\SetKwInOut{Input}{input}
\SetKwInOut{Output}{output}
\Input{$op$: operator $group\_size$: (30, ... 1) \\
$P, N, U$: pos/neg/undecidable tags\\
}
\Output{$P, N, U$ (updated)}

$Q$ $\gets$ initialize upload queue\\
%$groups$ $\gets$ divide the query time range into groups based on $window\_size$\\
$groups$ $\gets$ divide the query time range into groups \\
\For(\tcp*[h]{rapid attempting}){$g$ in $groups$}{
	\lIf{any frame in $g$ is $P$/$N$}{
		pass
	}
	\lElseIf{any frame in $g$ is $U$}{
		add frame to $Q$
	}
	\uElse{
		$f$ $\gets$ pick a random frame from $g$\\
		process and tag $f$ with $op$\\
		\lIf{$f$ tagged as $U$}{
			add $f$ to $Q$
		}
	}
}
\While(\tcp*[h]{work stealing}){$Q$ is not empty}{
	$f \gets Q$.tail(); $g$ $\gets$ enclosing group of $f$ \\
	$f1$ $\gets$ an untagged frame within $g$ \\
	process and tag $f1$ with $op$ \\
	\lIf{$f1$ tagged as $P$/$N$}{
		remove $f$ from $Q$
	}
}
\end{algorithm}
%\vspace{-10pt}
\end{comment}



==> schedule.tex <==
% !TeX root = main.tex
\section{Jointly deciding tile sizes and scheduling IO/compute tasks in parallel}

%\section{Scheduling IO/compute tasks in parallel}
In order to reduce IO overhead in swapping, \sys{} automatically overlaps IO tasks and compute tasks across layers and frames based on NN characteristics.

\begin{comment}
\begin{table*}[t]
	\centering
	\begin{adjustbox}{max width=1.\textwidth,center}
	\begin{tabular}{c|c|c|c|c|c}
		\hline 
		Tile & tile size & \# of tiles & IO (r/w) time & compute time & description\\
		\hline
		input 	& tsize\_in 	& 1 	& 1 * rtime\_in 	& 0				& read 1 tile \\ 
		\hline
		weight 	& tsize\_wt		& N 	& N * rtime\_wt 	& N * ctime\_wt & read N tiles, compute N times for sub-channels of output \\
		\hline
		output 	& tsize\_out 	& 1		& 1 * wtime\_out 	& 0 			& write 1 tile\\
		\hline
	\end{tabular}
	\end{adjustbox}
	\caption{Properties of IO/compute tasks for computing every single output tile: (2 + N) * IO-tasks + N * compute-tasks, where N is the number of weight tiles. }
	\label{tab:task-property}
\end{table*}
\end{comment}

\subsection{Challenges and solution}
\paragraph{Parallel scheduling}
As shown in Figure~\ref{fig:swap-model}, MCU ideally could extract CPU/IO parallelism for hiding IO delays.
However, such ideal parallel scheduling sequence is difficult to find because it must meet the following requirements at the same time:
(1) the scheduler must automatically identify what tiles should be executed in parallel according to their dependencies and relative IO/compute time;
(2) the working set of tiles being executed in parallel must be smaller than SRAM at every single moment;
(3) the parallel sequence should keep both MCU core and IO bandwidth fully utilized to avoid either of them from idling.

\paragraph{Deciding tile sizes}
Tile sizes affect swapping performance and they are difficult to decide.
If tile sizes are too large, the tiles that should be executed in parallel to overlap IO/compute time cannot be executed in parallel because their working set is larger than SRAM size, leading to low parallelism.
In contrast, if tile sizes are too small, the overhead of synchronizing/issuing more short IO/compute tasks is high, leading to low performance and non-efficient MCU/memory utilization. 
Therefore, it's hard to automatically find appropriate tile sizes for all layers, especially when tiles' co-existing is hard to predict due to the uncertainty of parallel execution.

Divers NN layers with different parameters and diverse SRAM sizes on MCUs create a huge space for deciding parallel sequence of IO/compute tasks and tile sizes, so it's hard to automatically find the optimal configuration that can perfectly overlap IO/compute tasks across layers/frames to reduce the IO overhead in swapping.

\paragraph{Solution}
We design an system to jointly decide tile sizes and find the optimal parallel sequences for IO/compute tasks, since they are related to each other and cannot be decide separately.
The system consists of two components:
(1) a scheduling planner that can find the optimal parallel sequence for IO/compute tasks across layers/frames based on given tile sizes and SRAM size.
(2) a searching algorithm that jointly finds the best tile sizes and parallel sequences by enumerating possible tile sizes based on the scheduling planner in (1) (how to do better? time complexity?). 

Design goals:???

\subsection{Scheduler}
\input{fig-scheduler.tex}

\paragraph{Defining NN tasks}
As shown in Table~\ref{tab:task-property}, \sys{} defines two types of tasks: IO tasks and Compute tasks.
An IO task reads an input/weight tile from SD or writes an output tile to SD, and its properties include tile size and IO time.
An IO task is ready to be executed only if the memory buffer for input/weight tile is successfully allocated or the output tile has been computed.
A compute task computes an output tile based on corresponding input tile and weight tiles, and its properties include input/weight/output tile sizes and compute time.
A compute task is ready to be executed only if its input/weight tiles are already in SRAM and the memory buffer for output tile has already been successfully allocated.


\paragraph{Graphs of NN tasks}
%Different from traditional computation graphs~\cite{ding2020ios} that define computation operators as nodes and dependencies as edges, 
%\sys{} defines both IO and compute tasks as nodes and their dependencies as edges, as shown in Figure~\ref{fig:scheduler}.
\sys{} define CNN as a computation graph \textit{G = (V, E)}, 
where V is the node set of IO and Compute tasks, and E is the edge set representing dependencies.
For instance, a compute task depends on two IO tasks that read input/weight tiles, and a write IO depends on N compute tasks that compute all channels of an output tile.  
It is worth nothing that we enforce dependencies between an input tile and multiple weight tiles to ensuring reading input tile first, 
so that reading other weight tiles can happen in parallel with computing an output tile.

\paragraph{Task state}
As shown in Figure~\ref{fig:scheduler}, \sys{} define the following states for every IO/Compute task:
\begin{itemize}
	\item \textbf{INIT} A task is set to INIT state when building the execution graph based on NN architecture and tiling configurations.
	 
	\item \textbf{READY} A task becomes READY when: 
	(1) all of its predecessors have finished, at which point the \textit{in-degree counter} of the task drops to zero;
	(2) the memory buffer has been successfully allocated, e.g., the memory buffers of input/weight tile for a read IO, the output buffer for a Compute task.
	%(1) for read IO, all of its predecessors have finished and the memory for reading data has been allocated;
	%(2) for write IO, all of its predecessors have finished;
	%(3) for Compute tasks, its all predecessors have finished and the memory buffer for output tile has been allocated.
	  
	\item \textbf{SELECTED} \sys{} selects a small set of IO/compute tasks in READY states to execute in parallel based on their priority and MCU/IO utilization, and \sys{} sets them into SELECTED state.
	
	\item \textbf{FINISHED} When a IO/compute task is finished, it switches to FINISHED state, at which point \sys{} will decrease the \textit{in-degree counter} by one for this task's successors to release the dependency and free memory buffers.
	
\end{itemize}

\paragraph{Scheduling NN tasks}
Given a tiling strategies of NN layers, \sys{} finds the optimal parallel sequences for IO and compute tasks based on their dependencies and SRAM sizes.
One goal of scheduling is to keep both MCU and IO busy to avoid either of them from idling for high system throughput.
\sys{} schedules IO tasks based on available memory space to pre-load tiles for future compute tasks, and timely write back and free space for completed tiles.
\sys{} schedules compute tasks based on their input dependencies and task priority, which ensures that tasks from early frames will higher priority to be schedule for per-frame latency.

There are two constraints in scheduling: available SRAM buffer sizes and task dependencies.
The goal of scheduling is to keep both MCU and IO busy by maximizing the overlapping of compute and IO tasks.

The pseudo code of building graph and scheduling tasks is shown in Algorithm ~\ref{algo:scheduler}. 


\input{schedule-algorithm}


\subsection{Searching algorithm}
The pseudo code of searching algorithm is shown in Algorithm~\ref{algo:search}.
\input{search-algorithm}


\subsection{Time complexity of search algorithm}
%What's the time complexity? How to reduce the complexity?
Given the tiny SRAM size and slow MCU, the co-existing tiles won't be too many (2 to 3 layers at most) and the possible tile size for each layer is limited, because there are only two cases for each layer: executed alone, and executed in parallel with other layers.
The working set of a layer is 1/2 (1/2 compute, 1/2 for next tiles IO) of memory buffer if the layer will be executed alone, and is 1/4 memory buffer if it's co-executed in parallel with other layers. 
So the possible tile sizes for a NN is limited and can be calculated on server/desktop before deployment.


==> search-algorithm.tex <==
% !TeX root = main.tex
\begin{algorithm}
\small
%\SetAlgoLine
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{NN architecture and SRAM size}
\Output{Tile sizes and parallel IO/compute sequence }

%Let $tsIn[i]$, $tsWt[i]$, $tsOut[i]$= input, weight, output tile sizes of layer $i$\\
Let $Layers[L]$ = $L$ layers of an NN \\
Let $TileConfig[T]$ = possible tile size configurations ($T$ in total)

\SetKwFunction{FSearch}{Search}
    \SetKwProg{Fn}{Function}{:}{}
    \Fn{\FSearch{$Layers$, $MemSize$}}{
    $minTime \longleftarrow$ MAX\_INT; \\
    $bestTileConfig \longleftarrow$ NULL; \\
    \For{$tconfig \in TileConfig$} {
	    $timeBegin \longleftarrow$ currentTime(); \\
		// can find best sequence with only 3 frames \\
		$G1 \longleftarrow BuildGraph(Layers, tconfig, time1)$; \\
		$G2 \longleftarrow BuildGraph(Layers, tconfig, time2)$; \\
		$G3 \longleftarrow BuildGraph(Layers, tconfig, time3)$; \\
		\While{!ReadyIO.empty || !ReadyCP.empty} {
			$SelectTask$ ($ReadyIO$, $ReadyCP$, $SelectedIO$, $SelectedCP$); \\
			$ScheduleTask$ ($SelectedIO$, $SelectedCP$);
		}
		$timeEnd \longleftarrow$ currentTime(); \\
		\If{$timeEnd - timeBegin < minTime$} {
			$bestTileConif \longleftarrow tconfig$; \\
			$minTime = timeEnd - timeBegin$;
		}
    }
	\textbf{return} $bestTileConfig$;
}
\textbf{End Function}
\caption{Jointly search tile size and parallel sequence jointly}
\label{algo:search}
\end{algorithm}


\begin{comment}
\begin{algorithm}
\small
%\SetAlgoLine
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{NN architecture and SRAM size}
\Output{Tile sizes and parallel IO/compute sequence }

\texttt{\\} % add a blank line

%Let $tsIn[i]$, $tsWt[i]$, $tsOut[i]$= input, weight, output tile sizes of layer $i$\\
Let $Layers[L]$ = $L$ layers of an NN \\
Let $tnIn[L]$, $tnWt[L]$, $tnOut[L]$ = number of input, weight, and output tiles of NN layers \\

Let $\longrightarrow$ = add a task to graph to create dependency and update $inDegreeCounter$ for each task

\SetKwFunction{FBuildGraph}{BuildGraph}
    \SetKwProg{Fn}{Function}{:}{}
    \Fn{\FBuildGraph{$Layers$, $tIn$, $tWt$, $tOut$}}{
	    $G$ = empty graph \\
	    \For{$Layer \in Layers$} {
		    \For{$tin \in tIn$} {
				$IOTask\_ReadInput \longrightarrow G$; \\
				\For{$twt \in tWt$} {
					$IOTask\_ReadWt \longrightarrow G$; \\
					$ComputeTask \longrightarrow G$; \\
				}
		    }
		    $IOTask\_WriteOutput \longrightarrow G$;
	    }
	    Set the root IOTask to READY and insert into $ReadyIO$; \\
        \textbf{return} $G;$ 
}
\textbf{End Function}
\caption{Jointly search tile size and parallel sequence jointly}
\label{algo:search}
\end{algorithm}
\end{comment}

==> swap-model.tex <==

%\begin{figure}[t!]
\begin{figure*}
\centering
    \includegraphics[width=0.95\textwidth{}]{./figs/swap-model} 
    \caption{System overview: showing Convolutional (compute-bound) and Fullyconected (IO-bound) layer.}
    %\vspace{-2pt}		% use as needed
    \label{fig:swap-model}
\end{figure*}

